Selectively-Amortized Resource Bounding (Extended Version)

We consider the problem of automatically proving resource bounds. That is, we study how to prove that an integer-valued resource variable is bounded by a given program expression. Automatic resource-bound analysis has recently received significant attention because of a number of important applications (e.g., detecting performance bugs, preventing algorithmic-complexity attacks, identifying side-channel vulnerabilities), where the focus has often been on developing precise amortized reasoning techniques to infer the most exact resource usage. While such innovations remain critical, we observe that fully precise amortization is not always necessary to prove a bound of interest. And in fact, by amortizing selectively, the needed supporting invariants can be simpler, making the invariant inference task more feasible and predictable. We present a framework for selectively-amortized analysis that mixes worst-case and amortized reasoning via a property decomposition and a program transformation. We show that proving bounds in any such decomposition yields a sound resource bound in the original program, and we give an algorithm for selecting a reasonable decomposition.

==> bectex/Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = main
PAPERS = $(BASE)

# Generate short bib
%.short.bib: %.orig.bib
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/^[ 	]*[Ee]ditor/OPTeditor/' \
            -e 's/^[ 	]*[Mm]onth/OPTmonth/' \
            -e 's/^[ 	]*[Pp]ublisher/OPTpublisher/' \
            -e 's/^[ 	]*[Aa]ddress/OPTaddress/' \
            -e 's/^[ 	]*[Ii]sbn/OPTisbn/' \
            -e 's/^[ 	]*[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/^[ 	]*[Dd]oi/OPTdoi/' \
            -e 's/^[ 	]*[Pp]ages/OPTpages/' \
            -e 's/^[ 	]*[Cc]rossref/OPTcrossref/' \
            -e 's/^[ 	]*[Ss]eries/OPTseries/' \
            $< > $@
						
include bectex.mk


==> proof-cmd.tex <==
\begin{figure}[!tb]
\scriptsize

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-UBCheck}. Without loss of generality, let $\orig \cmd = \ubassert{\resvar}{\expr}$ and $\cmd = \ubassert{\decomp(\orig \resvar)}{\expr}$, prove there exists $\orig \pstore'$ such that $\evalcmd{\orig \pstore}{ \ubassert{\resvar}{\expr} }{ \orig \pstore' }$.
  Assume: (1) there exists number $n_1$ such that $\evalexpr{\orig \pstore}{\expr}{n_1}$, (2) there exists number $n_2$ such that $\evalexpr{\pstore}{\expr}{n_2}$.
]{
\begin{mathpar}
\inferrule*[vcenter, Right={\tiny E-UBCheck}]{
  \evalexpr{\orig \pstore}{\expr}{n_1}
  \\
  \inferrule*[vcenter, ]{
    \inferrule*[vcenter, ]{
      \text{Premise 1}
      \\
      \text{Premise 2}
    }{
      \pstore(\orig \resvar)
      \leq n_1
    }
  }{
    \left(\Sum_{\resvar \in \{ \orig \resvar \}}
    \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)\right)
    \leq n_1
  }
}{
  \evalcmd{\orig \pstore}{ \ubassert{\resvar}{\expr} }{ \orig \pstore }
}
\\\\
\inferrule*[vcenter, Lab={\rm\scriptsize Premise 1:}, Right={\tiny {\rm Based on} E-UBCheck}]{
  \evalcmd{\pstore}{\ubassert{\decomp(\orig \resvar)}{\expr}}{\pstore'}
  \\
  \evalexpr{\pstore}{\expr}{n_2}
}{
  \left(\Sum_{\resvar \in \decomp(\orig \resvar)}
  \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)\right)
  \leq n_2
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 2:}, Right={\tiny {\rm By definition}}]{
  \samevarstore{\orig \pstore}{\pstore}
}{
  \orig\pstore(\orig\resvar)
  \leq
  \Sum_{\resvar \in \decomp(\orig\resvar)} \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)
  \\
  \inferrule*[vcenter, ]{
    \orig\pstore(\var) = \pstore(\var) \text{ for all } \var \in \Vars(\orig\pstore) = \Vars(\pstore)
    \\\\
    \evalexpr{\orig \pstore}{\expr}{n_1}
    \\
    \evalexpr{\pstore}{\expr}{n_2}
  }{
    n_1 = n_2
  }
}
\end{mathpar}
}

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-Use}. Without loss of generality, let  $\orig \cmd = \auxupdate{\orig \resvar}{\expr}$ and $\cmd = \auxupdate{\resvar}{\expr}$ for some $\resvar \in \decomp(\orig \resvar)$, prove there exists $\orig \pstore'$ such that $\evalcmd{\orig \pstore}{ \auxupdate{\orig \resvar}{\expr} }{ \orig \pstore' }$.
]{
\begin{mathpar}
\inferrule*[vcenter, Right={\tiny E-Use}]{
  \evalexpr{\orig \pstore}{\expr}{\valn}
}{
  \evalcmd{\orig \pstore}{ \auxupdate{\orig \resvar}{\expr} }{ \mapext{\pstore}{\orig \resvar}{\pstore(\orig \resvar) + \valn} }
}
\end{mathpar}
}

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-Reset}. Without loss of generality, let  $\orig \cmd = \cmdskip$ and $\cmd = \reset{\resvar'}$ for some $\resvar \in \decomp(\orig \resvar)$, prove there exists $\orig \pstore'$ such that $\evalcmd{\orig \pstore}{ \cmdskip }{ \orig \pstore' }$.
]{
\begin{mathpar}
\inferrule*[vcenter, ]{
}{
  \evalcmd{\orig \pstore}{ \cmdskip }{ \orig \pstore }
}
\end{mathpar}
}

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-Command}. Prove there exists $\orig \pstore'$ such that $\evalcmd{\orig \pstore}{ \cmd }{ \orig \pstore' }$ when $\cmd \in \Set{ \cmdskip, \assign{\var}{\expr}, \assume{\expr}}$.
]{
\begin{mathpar}
\inferrule*[vcenter, ]{
  \evalcmd{\pstore}{\cmd}{\pstore'}
  \\
  \cmd \in \Set{ \cmdskip, \assign{\var}{\expr}, \assume{\expr}}
}{
  \evalcmd{\orig \pstore}{\cmd}{\orig \pstore'}
}
\end{mathpar}
}

\caption{Proof of \autoref{thm:sound-cmd} (Part 1): When the premises in \autoref{thm:sound-cmd} are met, prove there exists $\orig \pstore'$ such that $\evalcmd{\orig \pstore}{ \orig \cmd }{ \orig \pstore' }$.}
\label{fig:sound-cmd-1}
\end{figure}


\begin{figure}[!tb]
\scriptsize

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-UBCheck}. Without loss of generality, let $\orig \cmd = \ubassert{\resvar}{\expr}$ and $\cmd = \ubassert{\decomp(\orig \resvar)}{\expr}$, prove $\samevarstore{\orig{\pstore'}}{\pstore'}$.
]{
\begin{mathpar}
\inferrule*[vcenter, ]{
  \text{Premise 1}
  \\
  \text{Premise 2}
}
{
  \samevarstore{\orig{\pstore'}}{\pstore'}
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 1:}]{
  \inferrule*[vcenter, Right={\tiny {\rm By definition}}]{
    \samevarstore{\orig{\pstore}}{\pstore}
  }{
    \orig\pstore(\var) = \pstore(\var) \text{ for all } \var \in \Vars(\orig\pstore) = \Vars(\pstore)
  }
  \\
  \inferrule*[vcenter, Right={\tiny {\rm Based on} E-UBCheck}]{
    \evalcmd{\orig \pstore}{\ubassert{\resvar}{\expr}}{\orig \pstore'} \text{ (From \autoref{fig:sound-cmd-1})}
  }{
    \orig \pstore = \orig \pstore'
  }
  \qquad\qquad\qquad\qquad
  \inferrule*[vcenter, Right={\tiny {\rm Based on} E-UBCheck}]{
    \evalcmd{\pstore}{\ubassert{\decomp(\orig \resvar)}{\expr}}{\pstore'}
  }{
    \pstore = \pstore'
  }
}{
  \orig\pstore'(\var) = \pstore'(\var) \text{ for all } \var \in \Vars(\orig\pstore') = \Vars(\pstore')
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 2:}]{
  \inferrule*[vcenter, Right={\tiny {\rm By definition}}]{
    \samevarstore{\orig{\pstore}}{\pstore}
  }{
    \orig\pstore(\orig\resvar)
    \leq
    \Sum_{\resvar \in \decomp(\orig\resvar)} \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)
  }
  \\
  \inferrule*[vcenter, Right={\tiny {\rm Based on} E-UBCheck}]{
    \evalcmd{\orig \pstore}{\ubassert{\resvar}{\expr}}{\orig \pstore'} \text{ (From \autoref{fig:sound-cmd-1})}
  }{
    \orig \pstore = \orig \pstore'
  }
  \qquad\qquad\qquad\qquad
  \inferrule*[vcenter, Right={\tiny {\rm Based on} E-UBCheck}]{
    \evalcmd{\pstore}{\ubassert{\decomp(\orig \resvar)}{\expr}}{\pstore'}
  }{
    \pstore = \pstore'
  }
}{
  \orig\pstore'(\orig\resvar)
  \leq
  \Sum_{\resvar \in \decomp(\orig\resvar)} \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
}
\end{mathpar}
}

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-Use}. Without loss of generality, let  $\orig \cmd = \auxupdate{\orig \resvar}{\expr}$ and $\cmd = \auxupdate{\resvar}{\expr}$ for some $\resvar \in \decomp(\orig \resvar)$, prove $\samevarstore{\orig{\pstore'}}{\pstore'}$.
  Assume: (1) there exists number $n_1$ such that $\evalexpr{\orig \pstore}{\expr}{n_1}$, (2) there exists number $n_2$ such that $\evalexpr{\pstore}{\expr}{n_2}$.
]{
\begin{mathpar}
\inferrule*[vcenter, ]{
  \text{Premise 1}
  \\
  \text{Premise 2}
  \\
  \text{Premise 3}
  \\
  \text{Premise 4}
}{
  \orig\pstore'(\orig\resvar)
  \leq
  \Sum_{\resvar \in \decomp(\orig\resvar)} \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 1:}]{
  \samevarstore{\orig{\pstore}}{\pstore}
}{
  \orig\pstore(\orig\resvar)
  \leq
  \Sum_{\resvar \in \decomp(\orig\resvar)} \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 2:}]{
  \evalcmd{\orig \pstore}{\expr}{n_1}
}{
  n_1 = \orig\pstore'(\orig\resvar) - \orig\pstore(\orig\resvar)
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 3:}]{
  \evalcmd{\pstore}{\expr}{n_2}
}{
  n_2 =
  \left(
    \Sum_{\resvar \in \decomp(\orig\resvar)}
    \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
  \right) -
  \left(
    \Sum_{\resvar \in \decomp(\orig\resvar)}
    \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)
  \right)
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 4:}]{
  \inferrule*[vcenter, ]{
    \samevarstore{\orig{\pstore}}{\pstore}
  }{
    \orig\pstore(\var) = \pstore(\var) \text{ for all } \var \in \Vars(\orig\pstore) = \Vars(\pstore)
  }
  \\
  \evalcmd{\orig \pstore}{\expr}{n_1}
  \\
  \evalcmd{\pstore}{\expr}{n_2}
}{
  n_1 = n_2
}

\inferrule*[vcenter, ]{
  \inferrule*[vcenter, ]{
    \samevarstore{\orig{\pstore}}{\pstore}
  }{
    \orig\pstore(\var) = \pstore(\var) \text{ for all } \var \in \Vars(\orig\pstore) = \Vars(\pstore)
  }
  \\
  \inferrule*[vcenter, Right={\tiny E-Use}]{
    \evalexpr{\orig \pstore}{\expr}{\valn}
  }{
    \evalcmd{\orig \pstore}{ \auxupdate{\resvar}{\expr} }{ \mapext{\orig \pstore}{\resvar}{\orig \pstore(\resvar) + \valn} }
  }
  \\
  \inferrule*[vcenter, Right={\tiny E-Use}]{
    \evalexpr{\pstore}{\expr}{\valn}
  }{
    \evalcmd{\pstore}{ \auxupdate{\resvar}{\expr} }{ \mapext{\pstore}{\resvar}{\pstore(\resvar) + \valn} }
  }
}{
  \orig\pstore'(\var) = \pstore'(\var) \text{ for all } \var \in \Vars(\orig\pstore') = \Vars(\pstore')
}
\end{mathpar}
}

\caption{Proof of \autoref{thm:sound-cmd} (Part 2.1): When the premises in \autoref{thm:sound-cmd} are met, prove $\samevarstore{\orig{\pstore'}}{\pstore'}$ when $\hypdecomp{\orig\cmd}{\cmd}$ is \TirName{D-UBCheck} or \TirName{D-Use}.}
\label{fig:sound-cmd-2}
\end{figure}


\begin{figure}[!tb]
\scriptsize

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-Reset}. Without loss of generality, let  $\orig \cmd = \cmdskip$ and $\cmd = \reset{\resvar'}$ for some $\resvar \in \decomp(\orig \resvar)$, prove $\samevarstore{\orig{\pstore'}}{\pstore'}$.
]{
\begin{mathpar}

\inferrule*[vcenter, ]{
  \inferrule*[vcenter, Right={\tiny {\rm Semantics of $\cmdskip$}}]{
    \\
  }{
    \orig \pstore(\orig \resvar) = \orig \pstore'(\orig \resvar)
  }
  \qquad\qquad\qquad\qquad
  \text{Premise 1}
}{
  \orig \pstore'(\orig \resvar) \le
  \left(
    \Sum_{\resvar \in \decomp(\orig\resvar)}
    \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
  \right)
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 1:}]{
  \text{Premise 2 is true for any $\resvar$ such that $\resvar \in \decomp(\orig \resvar) \land \resvar = \resvar'$}
  \\
  \text{Premise 3 is true for any $\resvar$ such that $\resvar \in \decomp(\orig \resvar) \land \resvar \ne \resvar'$}
}{
  \inferrule*[vcenter, ]{
    \text{For any $\resvar$ such that $\resvar \in \decomp(\orig \resvar)$: }
    \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)
    \le
    \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
  }{
    \left(
      \Sum_{\resvar \in \decomp(\orig\resvar)}
      \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)
    \right) \le \left(
      \Sum_{\resvar \in \decomp(\orig\resvar)}
      \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
    \right)
  }
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 2:}, Right={\tiny E-Reset}]{
  \pstore'(\cnt{\resvar}) = \pstore(\cnt{\resvar}) + 1
  \\
  \pstore'(\ub{\resvar}) = \max(\pstore(\ub{\resvar}), \pstore(\resvar))
  \\
  \pstore'(\resvar) = 0
}{
  \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar) \le \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 3:}, Right={\tiny E-Reset}]{
  \pstore'(\cnt{\resvar}) = \pstore(\cnt{\resvar})
  \\
  \pstore'(\ub{\resvar}) = \pstore(\ub{\resvar})
  \\
  \pstore'(\resvar) = \pstore(\resvar)
}{
  \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar) = \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
}

\inferrule*[vcenter, ]{
  \inferrule*[vcenter, ]{
    \samevarstore{\orig{\pstore}}{\pstore}
  }{
    \orig\pstore(\var) = \pstore(\var) \text{ for all } \var \in \Vars(\orig\pstore) = \Vars(\pstore)
  }
  \\
  \inferrule*[vcenter, Right={\tiny E-Reset}]{
    \pstore' =
    \mapext{
      \mapext{
        \mapext{
          \pstore}
              {\cnt{\resvar}}{ \pstore(\cnt{\resvar}) + 1}
      }
            {
              \ub{\resvar}}{ \max(\pstore(\ub{\resvar}), \pstore(\resvar))
            }
    }{\resvar}{0}
  }{
    \evalcmd{\pstore}{ \reset{\resvar} }{ \pstore' }
  }
}{
  \orig\pstore'(\var) = \pstore'(\var) \text{ for all } \var \in \Vars(\orig\pstore') = \Vars(\pstore')
}
\end{mathpar}
}

\subfloat[
  When $\hypdecomp{\orig\cmd}{\cmd}$, consider \TirName{D-Command}. Prove $\samevarstore{\orig{\pstore'}}{\pstore'}$.
  This derivation tree is valid for any command $\cmd$ and $\orig \cmd$ such that $\cmd = \orig \cmd$ and $\cmd \in \Set{ \cmdskip, \assign{\var}{\expr}, \assume{\expr}}$.
]{
\begin{mathpar}
\inferrule*[vcenter, ]{
  \text{Premise 1}
  \\
  \text{Premise 2}
}
{
  \samevarstore{\orig{\pstore'}}{\pstore'}
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 1:}]{
  \inferrule*[vcenter, Right={\tiny {\rm By definition}}]{
    \samevarstore{\orig{\pstore}}{\pstore}
  }{
    \orig\pstore(\var) = \pstore(\var) \text{ for all } \var \in \Vars(\orig\pstore) = \Vars(\pstore)
  }
  \qquad\qquad\qquad\qquad
  \inferrule*[vcenter, ]{
    \evalcmd{\orig \pstore}{\cmd}{\orig \pstore'}
  }{
    \orig \pstore = \orig \pstore'
  }
  \\
  \inferrule*[vcenter, ]{
    \evalcmd{\pstore}{\cmd}{\pstore'}
  }{
    \pstore = \pstore'
  }
}{
  \orig\pstore'(\var) = \pstore'(\var) \text{ for all } \var \in \Vars(\orig\pstore') = \Vars(\pstore')
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 2:}]{
  \inferrule*[vcenter, Right={\tiny {\rm By definition}}]{
    \samevarstore{\orig{\pstore}}{\pstore}
  }{
    \orig\pstore(\orig\resvar)
    \leq
    \Sum_{\resvar \in \decomp(\orig\resvar)} \pstore(\cnt{\resvar}) \cdot \pstore(\ub{\resvar}) + \pstore(\resvar)
  }
  \qquad\qquad\qquad\qquad
  \inferrule*[vcenter, ]{
    \evalcmd{\orig \pstore}{\cmd}{\orig \pstore'}
  }{
    \orig \pstore = \orig \pstore'
  }
  \\
  \inferrule*[vcenter, ]{
    \evalcmd{\pstore}{\cmd}{\pstore'}
  }{
    \pstore = \pstore'
  }
}{
  \orig\pstore'(\orig\resvar)
  \leq
  \Sum_{\resvar \in \decomp(\orig\resvar)} \pstore'(\cnt{\resvar}) \cdot \pstore'(\ub{\resvar}) + \pstore'(\resvar)
}
\end{mathpar}
}

\caption{Proof of \autoref{thm:sound-cmd} (Part 2.2): When the premises in \autoref{thm:sound-cmd} are met, prove $\samevarstore{\orig{\pstore'}}{\pstore'}$ when $\hypdecomp{\orig\cmd}{\cmd}$ is \TirName{D-Reset} or \TirName{D-Command}.}
\label{fig:sound-cmd-3}
\end{figure}

==> proof-path.tex <==
\begin{figure}[!tb]
\scriptsize

\begin{mathpar}
\inferrule*[vcenter, Left=\textcircled{1}, Right={\tiny D-Step}]{
  % \hypdecomp{\ptrace}{\ptrace'}
  \text{Premise 1}
  \\
  \ptraceok{\traceconsstate{\traceconscmd{\ptrace}{\pstore}{\cmd}}{\pstate_\diamond}}
  \\
  \samevarstore{\pstate_\star}{\pstate_\diamond}
}{
  \hypdecomp{
    \traceconsstate{\ptrace_\star}{\pstate_\star}
   }{
    \traceconsstate{\traceconscmd{\ptrace}{\pstore}{\cmd}}{\pstate_\diamond}
   }
}

\inferrule*[vcenter, Lab={\rm\scriptsize Premise 1:}, Left=\textcircled{2}, Right={\tiny D-AppendCommand}]{
  \inferrule*[vcenter, Left=\textcircled{4}, Right={\tiny D-Step}]{
    \hypdecomp{\ptrace_\vartriangle}{\ptrace}
    \quad
    \ptraceok{\traceconsstate{\ptrace}{\locstore{\loc}{\pstore}}}
    \\\\
    \samevarstore{\locstore{\loc_\vartriangle}{\pstore_\vartriangle}}{\locstore{\loc}{\pstore}}
  }{
    \hypdecomp{
      \traceconsstate{\ptrace_\vartriangle}{\locstore{\loc_\vartriangle}{\pstore_\vartriangle}}
    }{
      \traceconsstate{\ptrace}{\locstore{\loc}{\pstore}}
    }
  }
  \qquad\qquad
  \hypdecomp{\cmd_\vartriangle}{\cmd}
  \\
  \ptrace_\star = \traceconscmd{\ptrace_\vartriangle}{\pstore_\vartriangle}{\cmd_\vartriangle}
}{
  \hypdecomp{
    \ptrace_\star
  }{
    \traceconscmd{\ptrace}{\pstore}{\cmd}
  }
}
\end{mathpar}
\caption{Proof of \autoref{thm:sound-path} when a trace is in the form of $\traceconsstate{\traceconscmd{\ptrace}{\pstore}{\cmd}}{\pstate}$.}
\label{fig:sound-path}
\end{figure}

==> proof-prog.tex <==
\begin{figure}[!tb]
\scriptsize

\subfloat[
  Prove $\hypdecomp{
    \traceconsstate{\orig\ptrace}{\locstore{\loc'}{\orig\pstore'}}
  }{
    \traceconsstate{\ptrace}{\locstore{\loc'}{\pstore'}}
  }$.
  \label{fig:sound-prog-1}
]{
% \scriptsize
% \begin{mathpar}
% \inferrule*[vcenter, Right={\tiny D-Step}]{
%   \inferrule*[vcenter, Right={\tiny D-AppendCommand}]{
%     \hypdecomp{
%       \traceconsstate{\orig\ptrace}{\locstore{\orig\loc}{\orig\pstore}}
%     }{
%       \traceconsstate{\ptrace}{\locstore{\loc}{\pstore}}
%       \quad
%       \inferrule*[vcenter, Right={\tiny D-Transition ({\rm reversed})}]{
%         \hypdecomp{\orig\prog}{\prog}
%         \quad
%         \orig\loc = \loc
%         \quad
%         \orig\loc' = \loc'
%       }{
%         \hypdecomp{\orig\cmd}{\cmd}
%       }
%     }
%   }{
%     \hypdecomp{
%       \traceconscmd{\orig\ptrace}{\orig\pstore}{\orig\cmd}
%     }{
%       \traceconscmd{\ptrace}{\pstore}{\cmd}
%     }
%   }
%   \\
%   \inferrule*[vcenter, Right={\tiny Ok-Step}]{
%     \ptraceok{\traceconsstate{\ptrace}{\locstore{\loc}{\pstore}}}
%     \\
%     \evalcmd{\pstore}{\cmd}{\pstore'}
%   }{
%     \ptraceok{\traceconsstate{\traceconscmd{\ptrace}{\pstore}{\cmd}}{\locstore{\loc'}{\pstore'}}}
%   }
%   \qquad\qquad
%   \inferrule*[vcenter, Right={\tiny \autoref{thm:sound-cmd}}]{
%     \inferrule*[vcenter, Right={\tiny D-Step ({\rm reversed})}]{
%       \hypdecomp{\traceconsstate{\orig\ptrace}{\orig\pstate}}{\traceconsstate{\ptrace}{\pstate}}
%     }{
%       \hypdecomp{\orig\pstate}{\pstate}
%     }
%     \quad
%     \evalcmd{\pstore}{\cmd}{\pstore'}
%     \quad
%     \evalcmd{\orig\pstore}{\orig\cmd}{\orig\pstore'}
%   }{
%     \samevarstore{\locstore{\orig\loc'}{\orig\pstore'}}{\locstore{\loc'}{\pstore'}}
%   }
% }{
%   \hypdecomp{
%     \traceconsstate{\orig\ptrace}{\locstore{\loc'}{\orig\pstore'}}
%    }{
%     \traceconsstate{\ptrace}{\locstore{\loc'}{\pstore'}}
%    }
% }
% \end{mathpar}

\begin{mathpar}
\inferrule*[vcenter, Right={\tiny D-Step}]{
  \text{Premise 1}
  \\
  \text{Premise 2}
  \\
  \text{Premise 3}
}{
  \hypdecomp{
    \traceconsstate{\orig\ptrace}{\locstore{\loc'}{\orig\pstore'}}
   }{
    \traceconsstate{\ptrace}{\locstore{\loc'}{\pstore'}}
   }
}

\inferrule*[vcenter, Right={\tiny D-AppendCommand}, Lab={\rm\scriptsize Premise 1:}]{
  \hypdecomp{
    \traceconsstate{\orig\ptrace}{\locstore{\orig\loc}{\orig\pstore}}
  }{
    \traceconsstate{\ptrace}{\locstore{\loc}{\pstore}}
    \quad
    \inferrule*[vcenter, Right={\tiny {\rm Based on} D-Transition}]{
      \hypdecomp{\orig\prog}{\prog}
      \quad
      \orig\loc = \loc
      \quad
      \orig\loc' = \loc'
    }{
      \hypdecomp{\orig\cmd}{\cmd}
    }
  }
}{
  \hypdecomp{
    \traceconscmd{\orig\ptrace}{\orig\pstore}{\orig\cmd}
  }{
    \traceconscmd{\ptrace}{\pstore}{\cmd}
  }
}
\\\\
\inferrule*[vcenter, Right={\tiny Ok-Step}, Lab={\rm\scriptsize Premise 2:}]{
  \ptraceok{\traceconsstate{\ptrace}{\locstore{\loc}{\pstore}}}
  \\
  \evalcmd{\pstore}{\cmd}{\pstore'}
}{
  \ptraceok{\traceconsstate{\traceconscmd{\ptrace}{\pstore}{\cmd}}{\locstore{\loc'}{\pstore'}}}
}
\\
\inferrule*[vcenter, Right={\tiny \autoref{thm:sound-cmd}}, Lab={\rm\scriptsize Premise 3:}]{
  \inferrule*[vcenter, Right={\tiny {\rm Based on} D-Step}]{
    \hypdecomp{\traceconsstate{\orig\ptrace}{\orig\pstate}}{\traceconsstate{\ptrace}{\pstate}}
  }{
    \hypdecomp{\orig\pstate}{\pstate}
  }
  \qquad\qquad\qquad\qquad
  \evalcmd{\pstore}{\cmd}{\pstore'}
  \\
  \evalcmd{\orig\pstore}{\orig\cmd}{\orig\pstore'}
}{
  \samevarstore{\locstore{\orig\loc'}{\orig\pstore'}}{\locstore{\loc'}{\pstore'}}
}
\end{mathpar}
}

\subfloat[
  Prove $\ptraceok{\traceconsstate{\ptrace}{\locstore{\loc'}{\pstore'}}}$.
  \label{fig:sound-prog-2}
]{
\begin{mathpar}
\inferrule*[vcenter, Right={\tiny Ok-Step}]{
  \ptraceok{ \traceconsstate{\ptrace}{\locstore{\loc}{\pstore}} } \\
  \evalcmd{\pstore}{\cmd}{\pstore'}
}{
  \ptraceok{
    \traceconsstate{\traceconscmd{\ptrace}{\pstore}{\cmd}}{\locstore{\loc'}{\pstore'}} 
  }
}
\end{mathpar}
}
\caption{Proof of \autoref{lemma:sound-prog} in the inductive case.}
\end{figure}
